Search for Hydrogenated C$_{60}$ (fulleranes) in Circumstellar Envelopes

The recent detection of fullerene (C$_{60}$) in space and the positive assignment of five diffuse interstellar bands to C$_{60}^+$ reinforce the notion that fullerene-related compounds can be efficiently formed in circumstellar envelopes and be present in significant quantities in the interstellar medium. Experimental studies have shown that C$_{60}$ can be readily hydrogenated, raising the possibility that hydrogenated fullerenes (or fulleranes, C$_{60}$H$_m$, $m=1-60$) may be abundant in space. In this paper, we present theoretical studies of the vibrational modes of isomers of C$_{60}$H$_m$. Our results show that the four mid-infrared bands from the C$_{60}$ skeletal vibrations remain prominent in slightly hydrogenated C$_{60}$, but their strengths diminish in different degrees with increasing hydrogenation. It is therefore possible that the observed infrared bands assigned to C$_{60}$ could be due to a mixture of fullerenes and fulleranes. This provides a potential explanation for the observed scatter of the C$_{60}$ band ratios. Our calculations suggest that a feature around 15$\mu$m due to the breathing mode of heavily hydrogenated C$_{60}$ may be detectable astronomically. A preliminary search for this feature in 35 C$_{60}$ sources is reported.

==> bib.tex <==
%\begin{thebibliography}{}


\bibitem[Bern{\'e} et al.(2013)]{ber13} Bern{\'e}, O., Mulas, G., \& Joblin, C.\ 2013, \aap, 550, L4 

\bibitem[Bern{\'e} \& Tielens(2012)]{ber12} Bern{\'e}, O., \& Tielens, A.~G.~G.~M.\ 2012, PNAS, 109, 401 


\bibitem[Bernard-Salas et al.(2012)]{bc12} Bernard-Salas, J., Cami, J., Peeters, E., et al.\ 2012, \apj, 757, 41 

\bibitem[Bonchev \& Rouvray(1995)]{br95} Bonchev, D., \& Rouvray D. H.
\ 1995, Chemical Group Theory: Techniques and Applications,
Gordon and Breach Science Publishers 

\bibitem[Brieva et al.(2016)]{bg16} Brieva, A.~C., Gredel, R., J{\"a}ger, C., Huisken, F., \& Henning, T.\ 2016, \apj, 826, 122 

\bibitem[Cami et al.(2010)]{cami10}  Cami, J., Bernard-Salas, J., Peeters, E., \& Malek, S. E. 2010, Science, 329, 1180

\bibitem[Campbell et al.(2015)]{c15} Campbell, E.~K., Holz, M., Gerlich, D., \& Maier, J.~P.\ 2015, \nat, 523, 322 

\bibitem[Campbell et al.(2016a)]{c16a} Campbell, E.~K., Holz, M., \& Maier, J.~P.\ 2016a, \apjl, 826, L4 

\bibitem[Campbell et al.(2016b)]{c16b} Campbell, E.~K., Holz, M., Maier, J.~P., et al.\ 2016b, \apj, 822, 17 

\bibitem[Cataldo \& Iglesias-Groth(2009)]{ci09} Cataldo, F., \& Iglesias-Groth, S.\ 2009, \mnras, 400, 291 

\bibitem[Cataldo \& Iglesias-Groth(2010)]{ca10} Cataldo, F., \& Iglesias-Groth, S., 2010, Fulleranes: The Hydrogenated Fullerenes. Springer, Berlin

\bibitem[Cataldo et al.(2009)]{cs09} Cataldo, F., Strazzulla, G., \& Iglesias-Groth, S.\ 2009, \mnras, 394, 615 


\bibitem[D{\'{\i}}az-Luis et al.(2015)]{dg15} D{\'{\i}}az-Luis, J.~J., Garc{\'{\i}}a-Hern{\'a}ndez, D.~A., Kameswara Rao, N., Manchado, A., \& Cataldo, F.\ 2015, \aap, 573, A97 

\bibitem[D{\'{\i}}az-Luis et al.(2016)]{dg16} D{\'{\i}}az-Luis, J.~J., Garc{\'{\i}}a-Hern{\'a}ndez, D.~A., Manchado, A., \& Cataldo, F.\ 2016, \aap, 589, A5 


\bibitem[Evans et al.(2012)]{ev12} Evans, A., van Loon, J.~T., Woodward, C.~E., et al.\ 2012, \mnras, 421, L92 


\bibitem[Foing \& Ehrenfreund(1994)]{f94} Foing, B.~H., \& Ehrenfreund, P.\ 1994, \nat, 369, 296 


\bibitem[Frisch et al.(2009)]{fr09} Frisch, M. J., Trucks, G. W., Schlegel, J. B., et al. 2009, Gaussian 09, Revision C.01 (Wallingford, CT: Gaussian, Inc.)


\bibitem[Fulara et al.(1993)]{fj93} Fulara, J., Jakobi, M., \& Maier, J. P.
1993, CPL, 211, 227


\bibitem[Garc{\'{\i}}a-Hern{\'a}ndez et al.(2011a)]{gar11} Garc{\'{\i}}a-Hern{\'a}ndez, D.~A., Iglesias-Groth, S., Acosta-Pulido, J.~A., et al.\ 2011a, \apjl, 737, L30

\bibitem[Garc\'{i}a-Hern\'{a}ndez et al.(2011b)]{Garcia11}
Garc\'{i}a-Hern\'{a}ndez, D. A., Kameswara Rao. N., \& Lambert, D. L., 2011b, \apj, 729, 126


\bibitem[Garc{\'{\i}}a-Hern{\'a}ndez et al.(2010)]{gar10} Garc{\'{\i}}a-Hern{\'a}ndez, D.~A., Manchado, A., Garc{\'{\i}}a-Lario, P., et al.\ 2010, \apjl, 724, L39 


\bibitem[Garc{\'{\i}}a-Hern{\'a}ndez et al.(2012)]{gar12} Garc{\'{\i}}a-Hern{\'a}ndez, D.~A., Villaver, E., Garc{\'{\i}}a-Lario, P., et al.\ 2012, \apj, 760, 107 

\bibitem[Goldshleger \& Moravsky(1997)]{gm97} Goldshleger, N.~F., \& Moravsky, A.~P.\ 1997, Russian Chemical Reviews, 66, 323 

\bibitem[Gielen et al.(2011)]{gielen11} Gielen, C., Cami, J., Bouwman, J., Peeters, E., \& Min, M.\ 2011, \aap, 536, A54 

\bibitem[Herbig (2000)]{herbig00} Herbig, G. H. 2000, \apj, 542, 334

\bibitem[Iglesias-Groth(2007)]{ig07} Iglesias-Groth, S.\ 2007, \apjl, 661, L167 

\bibitem[Iglesias-Groth et al.(2012)]{ig12} Iglesias-Groth, S., Garc{\'{\i}}a-Hern{\'a}ndez, D.~A., Cataldo, F., \& Manchado, A.\ 2012, \mnras, 423, 2868 

\bibitem[Iglesias-Groth \& Esposito(2013)]{ig13} Iglesias-Groth, S., \& Esposito, M.\ 2013, \apjl, 776, L2 

\bibitem[Jensen(2001)]{je01} Jensen, F. 2001, JChPh, 115, 9113

\bibitem[Jensen(2002)]{je02} Jensen, F. 2002, JChPh, 116, 7372

\bibitem[Kroto et al.(1985)]{kroto}
Kroto, H. W., Heath, J. R., Obrien, S. C., Curl, R. F., \& Smalley, R. E. 1985, Nature, 318, 162

\bibitem[Kwok et al.(1989)]{kwo89}
Kwok, S., Volk, K., \& Hrivnak, B. J. 1989, \apj, 345, L51


\bibitem[Kwok et al.(2001)]{kwok2001}   Kwok, S., Volk, K., \& Bernath, P.  2001, \apj, 554, L87

\bibitem[Kwok(2004)]{kwok2004} Kwok, S.\ 2004, Nature, 430, 985

%\bibitem[Kwok(2016)]{k16} Kwok, S.\ 2016, \aapr, 24, 8 

\bibitem[Laury(2012)]{lc12} Laury, M. L., Carlson, M. J., \& Wilson, A. K. 2012, JCoCh, 33, 2380

\bibitem[Maltseva et al.(2015)]{mp15} Maltseva, E., Petrignani, A., Candian, A., et al.\ 2015, \apj, 814, 23 

\bibitem[Micelotta et al.(2012)]{mic12} Micelotta, E.~R., Jones, A.~P., Cami, J., et al.\ 2012, \apj, 761, 35 


\bibitem[Omont(2016)]{om16} Omont, A.\ 2016, \aap, 590, A52 

\bibitem[Otsuka et al.(2013)]{ots13} Otsuka, M., Kemper, F., Hyung, S., et al.\ 2013, \apj, 764, 77 

\bibitem[Otsuka et al.(2014)]{ots14} Otsuka, M., Kemper, F., Cami, J., Peeters, E., \& Bernard-Salas, J.\ 2014, \mnras, 437, 2577 


\bibitem[Otsuka et al.(2016)]{ots16} Otsuka, M., Kemper, F., Leal-Ferreira, M.~L., et al.\ 2016, \mnras, 462, 12 

\bibitem[Pauzat(2011)]{pa11} Pauzat, F.\ 2011, EAS Publications Series, 46, 75        

\bibitem[Pauzat et al.(1995)]{pt95} Pauzat, F., Talbi, D., \& Ellinger, Y.\ 1995, \aap, 293, 263 

\bibitem[Pauzat et al.(2010)]{pp10} Pauzat, F., Pilm{\'e}, J., Toulouse, J., \& Ellinger, Y.\ 2010, \jcp, 133, 054301   


\bibitem[Pogulay et al.(2004)]{pog2004}
Pogulay AV, et al. 2004 
%Ionization energies of the C60 fullerene and its hydrogenated derivatives C60H18 and C60H36 determined by electron ionization. 
International Journal of Mass Spectrometry 233(1–3):165%-172

\bibitem[Roberts et al.(2012)]{rs12} Roberts, K.~R.~G., Smith, K.~T., \& Sarre, P.~J.\ 2012, \mnras, 421, 3277 

\bibitem[R{\"u}chardt et al.(1993)]{ru93}
R{\"u}chardt C., Gerst, M., Ebenhoch, J. et al. 1993, Agnew. Chem. Int. Ed. Engl., 32, 584

\bibitem[Sadjadi et al.(2015)]{sz15} Sadjadi, S., Zhang, Y., \& Kwok, S.\ 2015, \apj, 801, 34 

\bibitem[Sellgren et al.(2010)]{sel10} Sellgren, K., Werner, M. W., Ingalls, J. G., Smith, J. D. T., Carleton, T. M.,
\& Joblin, C. 2010, \apj, 722, L54

\bibitem[Snow \& Seab (1989)]{snow89}  Snow, T. P., \& Seab, C. G. 1989, \aap, 213, 291

\bibitem[Strelnikov et al.(2015)]{str15} Strelnikov, D., Kern, B., \& Kappes, M.~M.\ 2015, \aap, 584, A55 

\bibitem[Volk et al.(1999)]{vol99}
Volk, K., Kwok, S., \& Hrivnak, B. J. 1999, \apj, 516, L99

\bibitem[Walker et al.(2015)]{wb15} Walker, G.~A.~H., Bohlender, D.~A., Maier, J.~P., \& Campbell, E.~K.\ 2015, \apjl, 812, L8 

\bibitem[Webster(1992)]{web92} Webster, A.\ 1992, \mnras, 257, 463 

\bibitem[Webster(1995)]{web95} Webster, A.\ 1995, \mnras, 277, 1555


\bibitem[Zhang \& Kwok(2011)]{zk11} Zhang, Y., \& Kwok, S.\ 2011, \apj, 730, 126 
\bibitem[Zhang \& Kwok(2013)]{zk13} Zhang, Y., \& Kwok, S.\ 2013, EP\&S, 65, 1069 

\bibitem[Zhang et al.(2010)]{zk10} Zhang, Y., Kwok, S., \& Hrivnak, B.~J.\ 2010, \apj, 725, 990 

\bibitem[Zerenturk \& Berber(2012)]{zb12} Zerenturk, A., \& Berber, S.\ 2012, Solid State Communications, 152, 1522 


\bibitem[Zinner(1998)]{zinner1998} Zinner, E. 1998, Annual Review of Earth and Planetary Sciences, 26, 147

\bibitem[Zvereva et al.(2011)]{Zvereva2011} Zvereva, E. E., Shagidullin, A. R., \&  Katsyuba, S. A. 2011, J. Phys. Chem. A , 115, 63

%\end{thebibliography}

